Learning Probabilistic Temporal Logic Specifications for Stochastic Systems

There has been substantial progress in the inference of formal behavioural specifications from sample trajectories, for example, using Linear Temporal Logic (LTL). However, these techniques cannot handle specifications that correctly characterise systems with stochastic behaviour, which occur commonly in reinforcement learning and formal verification. We consider the passive learning problem of inferring a Boolean combination of probabilistic LTL (PLTL) formulas from a set of Markov chains, classified as either positive or negative. We propose a novel learning algorithm that infers concise PLTL specifications, leveraging grammar-based enumeration, search heuristics, probabilistic model checking and Boolean set-cover procedures. We demonstrate the effectiveness of our algorithm in two use cases: learning from policies induced by RL algorithms and learning from variants of a probabilistic model. In both cases, our method automatically and efficiently extracts PLTL specifications that succinctly characterise the temporal differences between the policies or model variants.

==> smt-based.tex <==
\subsection{SMT-based Learning Algorithm}
\label{sec:sat-based}

Our approach to solving Problem~\ref{prob:pass-learning} is by reducing it to satisfiability problems in Satisfiability Modulo Theories (SMT) framework.
Specifically, we rely on the theory of Linear Real Arithmetic (LRA).


Our reduction of % solution to 
Problem~\ref{prob:pass-learning} to LRA relies on designing a formula $\propformula^{\sample}_n$ that enables the search for an PCTL formula of size at most $n$ that is consistent with a sample $\sample$. 
The formula $\propformula^{\sample}_n$ has the following properties:
\begin{enumerate}
	\item $\propformula^{\sample}_n$ is satisfiable if and only if there exists an PCTL formula of size at most $n$ that is consistent with $\sample$; and
	\item from a satisfying valuation of $\propformula^{\sample}_n$, one can easily extract a suitable PCTL formula of size at most $n$.
\end{enumerate}

%One can then design an iterative algorithm to search for a 

%One can then find a minimal, consistent PCTL formula: 
One can then iteratively search for a minimal,  consistent formula: for increasing values of $n$, %check the satisfiability of 
if $\propformula^{\sample}_n$ is satisfiable, extract a consistent PCTL formula.

%Based on the formula $\propformula^{\sample}_n$, one can design an iterative algorithm to search for a minimal, suitable PCTL formula: for increasing values of $n$, check the satisfiability of $\propformula^{\sample}_n$ and if satisfiable, extract an PCTL formula.

The formula $\propformula^{\sample}_n$ is defined as a conjunction of subformulas with distinct roles: $\propformula^{\sample}_n := \propformula^{\mathsf{str}}_n \wedge \propformula^{\mathsf{sem}}_n \wedge \propformula^{\mathsf{con}}_n$.
The subformula $\propformula^{\mathsf{str}}$ encodes the structure of the prospective PCTL formula $\Phi$.
The subformula $\propformula^{\mathsf{sem}}$ encodes that the correct semantics of PCTL is used to interpret the prospective PCTL formula on the given DTMCs. Finally, the subformula $\propformula^{\mathsf{con}}$ ensures that the prospective PCTL formula holds on the models in $P$ and not in the models in $N$.

We now describe the subformulas of $\propformula^{\sample}_n$ in detail.


\paragraph{Encoding the structure of PCTL formulas.}
The structure of an PCTL formula is symbolically encoded as a \emph{syntax DAG}. A syntax DAG of an PCTL formula is simply a syntax tree
in which the common nodes are merged. Figure~\ref{fig:syntax-dag} depicts an example of a syntax tree and %syntax 
DAG of an PCTL formula.

\begin{figure}
	\centering
	\begin{tikzpicture}
        \node (1) at (0, 0) {$\lor$};
        \node (2) at (.8, -1) {$\lP_{\geq 0.5}\lU$};
        \node (3) at (-.8, -1) {$\lP_{\ge 1}\lX$};
        \node (4) at (0, -2) {$p$};
        \node (5) at (1.6, -2) {$\lP_{\ge 0}\lG$};
        \node (6) at (1.6, -3) {$q$};
        \draw[->] (1) -- (2); 
        \draw[->] (1) -- (3);
        \draw[->] (2) -- (4);
        \draw[->] (2) -- (5);
        \draw[->] (3) -- (4);
        \draw[->] (5) -- (6);
        \node at (0.2,0.2) {6};
        \node at (1.4,-.65) {4};
        \node at (-.2,-.67) {5};
        \node at (0,-1.6)  {3};
        \node at (2.1,-1.7) {2};
        \node at (1.8,-2.7) {1};
	\end{tikzpicture}
    \caption{Syntax DAG with identifiers (indicated above nodes) of $(\lP_{\ge 1}\lX(p))\lor (\lP_{\ge 0.5}(p\lU(\lP_{\ge 0}\lG(q))))$.}
	\label{fig:syntax-dag}
\end{figure}


To conveniently encode the syntax DAG of an PCTL formula, we first fix a naming convention for its nodes. For a formula of size at most $n$, we assign to each of its nodes an identifier in $\brck{1,n}$ such that the identifier of each node is larger than those of its children, if applicable. Note that such a naming convention may not be unique.
 %Based on these identifiers, 
We then denote the sub-formula of $\Phi$ rooted at Node~$i$ as $\Phi[i]$. Thus, $\Phi[n]$ denotes the entire formula $\Phi$.

Next, to encode a syntax DAG symbolically, we introduce the following variables: 
\begin{itemize}
\item Boolean variables $x_{i,\lambda}$ for $i\in\brck{1,n}$, $\lambda\in \prop\cup\{\neg,\wedge,\lP_{\ge\circ}\lX,\lP_{\ge\circ}\lU \}$;
\item Boolean variables $l_{i,j}$ and $r_{i,j}$ for $i\in\brck{1,n}$ and $j\in\brck{1,i-1}$; and
\item Real variables $p_{i}$ for $i\in\brck{1,n}$; 
\end{itemize}

The variable $x_{i,\lambda}$ tracks the operator labeled in Node~$i$, meaning, $x_{i,\lambda}$ is set to true if and only if Node~$i$ is labeled with $\lambda$.
The variable $l_{i,j}$ (resp., $r_{i,j}$) tracks the left (resp., right) child of Node~$i$, meaning, $l_{i,j}$ (resp., $r_{i,j}$) is set to true if and only if the left (resp., right) child of Node~$i$ is Node~$j$.
The variable $p_{i}$ is relevant only if $x_{i,\bullet}$ is set to true for some operator with probabilistic quantifier $\bullet \in \{\lP_{\ge\circ}\lX,\lP_{\ge\circ}\lG,\lP_{\ge\circ}\lU\}$.
The variable $p_{i}$ tracks the probability bound of the operator, meaning $p_{i}$ is set to 
$p\in \real$ if and only if Node~$i$ has the probabilistic quantifier $\lP_{\ge p}$. 


To ensure that these variables encode a valid syntax DAG, we impose structural constraints similar to the ones proposed by Neider and Gavran~\cite{flie}.
For instance, the constraint below ensures that each node is labeled with a unique operator:
\[\Big[ \bigwedge_{i\in\brck{1,n}} \bigvee_{\lambda \in \Lambda} x_{i,\lambda} \Big] \land \Big[\bigwedge_{i\in\brck{1,n}} \bigwedge_{\lambda \neq \lambda' \in \Lambda} \lnot x_{i,\lambda} \lor \lnot x_{i,\lambda'}  \Big]\]
We impose similar constraints to ensure that each node has a unique left and right child.
The formula $\Omega^{\mathsf{str}}_n$ is simply the conjunction of all such structural constraints.

Based on a satisfying valuation $v$ of $\Omega^{\mathsf{str}}_n$, one can construct a unique PCTL formula: label each Node~$i$ with the operator $\lambda$ for which $v(x_{i,\lambda})=1$, mark the left (resp., right) child with Nodes $j$ (resp., $j'$) for which $v(l_{i,j})=1$ (resp., $v(r_{i,j'})=1$), and assign $\lP_{\ge p}$ as probabilistic quantifier if $v(p_{i})=p$.

\paragraph{Encoding the semantics of PCTL formulas.}
To symbolically encode the semantics of the prospective PCTL formula $\Phi$ for a given DTMC $C$, we rely on encoding the PCTL model-checking procedure developed in~\cite{DBLP:journals/fac/HanssonJ94}. 
The procedure involves calculating, for each sub-formula $\Phi'$ of $\Phi$, the set 
\[\Sat(\Phi') = \{s\in S \mid s\models \Phi'\}\] 
of the states of $\markov$ where $\Phi'$ holds.

We can now describe how to compute the set $\Sat(\Phi)$. It is done inductively on the structure of the PCTL formula $\Phi$ as follows:% for the different possible PCTL formulas are stated as follows:
\begin{align}
&\Sat(p) = \{ s \in S~|~p \in \ell(s) \}, \text{ for any }p\in \prop,\\
&\Sat(\Phi \wedge \Psi) = \Sat(\Phi) \cap \Sat(\Psi),\\
&\Sat(\neg\Phi) = Q \setminus \Sat(\Phi),\\
&\Sat(\lP_{\bowtie p}\lX\Phi) =\{ s ~|~\sum_{s'\in \Sat(\Phi)}  P(s,s') \bowtie p \},\\
&\Sat(\lP_{\bowtie p}(\Phi_1 \lU^{\leq k} \Phi_2)) = \{s~|~ \PM^{\markov}_{s}(s\models (\Phi_1 \lU^{\leq k} \Phi_2)) \bowtie p \}, \text{where}\\  
&\PM^{\markov}_{s}(s\models \Phi_1 \lU^{\leq k} \Phi_2) =
\begin{cases}
    1 & \text{if } s\models \Phi_2,\\
    0 & \text{if } s\not\models \Phi_1 \\
    0 & \text{if } s\not\models \Phi_2 \text{ and } n=0\\
    \sum_{s'\in S} P(s,s') \cdot \PM(s'\models \Phi_1 \lU^{\leq k-1} \Phi_2) & \text{otherwise.}
\end{cases}
\end{align}
\todo{Only considered >= for probabilities and bounded until for now}

Our goal is to symbolically encode the above-described computation. To do so, we introduce the propositional variables $y^{\markov}_{i,s}$ for each $i\in\brck{1,n}$, $s\in S$, $\markov\in \sample$ that track whether a state $s \in S$
belongs to $\Sat(\Phi[i])$ for a sub-formula $\Phi[i]$ of $\Phi$. 
That is, 
$y^{\markov}_{i,s}$ is set to true if and only if $\Phi[i]$ holds in state $s$, i.e. $s\in\Sat(\Phi[i])$.

We now ensure that the variables $y^{\markov}_{i,s}$ are set correctly using the following set of constraints that follow from the definition of $\Sat(\Phi[i])$.
\begin{align*}
    \bigwedge_{p \in \prop} \bigwedge_{i \in \brck{1,n}} \Big[ x_{i,p} \Rightarrow \bigwedge_{s\in S,\; p\in \ell(s)} y^{\markov}_{i,s} \; \wedge \bigwedge_{s\in S,\; p\notin \ell(s)} \neg y^{\markov}_{i,s} \Big]%\label{eq:prop}
    \\
    \bigwedge_{\substack{{i \in \brck{1,n}}\\{j,j' \in \brck{1,i-1}}}} \Big[ [x_{i,\wedge}\wedge l_{i,j}\wedge r_{i,j'}] \Rightarrow \bigwedge_{s\in S}\big[ y^{\markov}_{i,s} \Leftrightarrow [y^{\markov}_{j,s} \wedge y^{\markov}_{j',s}]\big]\Big]%\label{eq:and}
    \\
    \bigwedge_{\substack{{i \in \brck{1,n}}\\{j \in \brck{1,i-1}}}} \Big[ [x_{i,\neg}\wedge l_{i,j}] \Rightarrow \bigwedge_{s\in S}\big[ y^{\markov}_{i,s} \Leftrightarrow \neg y^{\markov}_{j,s'}\big]\Big]%\label{eq:not}
    \\
    \bigwedge_{\substack{{i \in \brck{1,n}}\\{j \in \brck{1,i-1}}}} \Big[ [x_{i,\lP_{\ge\circ}\lX}\wedge l_{i,j}] \Rightarrow \bigwedge_{s\in S}\big[ y^{\markov}_{i,s} \Leftrightarrow \sum_{s'\in \mathit{succ}(s)} P(s,s')\cdot y^{\markov}_{j,s'} \ge p_i %q \in \mathsf{Pre}_i(y^C_j)
    \big]\Big]%\label{eq:EX}
\end{align*}\todo{encoding that combines the syntactic and semantic search}

For the operator $\lP_{\ge\circ}\lU^{\leq k}$, we introduce intermediate variables $q^{\markov}_{i,s,k}$ for each $i\in\brck{1,n}$, $s\in S$, $\markov\in \sample$, and $k\in\brck{1,K}$ that track the probability measure $\PM^{\markov}_{s}(s\models\Phi[j] \lU^{\leq k} \Phi[j'])$.
\begin{align}
\bigwedge_{\substack{{i \in \brck{1,n}}\\{j,j' \in \brck{1,i-1}}}} \Big[ [x_{i,\lP_{\ge\circ}\lU^{\leq K}}\wedge l_{i,j}\wedge r_{i,j'}]\\ \Rightarrow \bigwedge_{s\in S}\big[ q^{\markov}_{i,s,k}\ge p_i \wedge q^{\markov}_{i,s,0} = y_{j',s}\big]\\
\ite(y^{\markov}_{j',s}, \bigwedge_{0<k\leq K} q^{\markov}_{i,s,k}=1,
\ite(\neg y^{\markov}_{j,s}, \bigwedge_{0<k\leq K} q^{\markov}_{i,s,k}=0,\
\bigwedge_{0<k\leq K}   q^{\markov}_{i,s,k} = \sum_{s'\in S} P(s,s')\cdot q^{\markov}_{j,s',k-1} ))]\big]\Big]%\label{eq:and}
\end{align}
In the above constraint, $\ite$ refers to the \emph{if-then-else} construct, which is typical syntactic sugar employed in several SMT solvers.
